UWFormer: Underwater Image Enhancement via a Semi-Supervised Multi-Scale Transformer

Underwater images often exhibit poor quality, distorted color balance and low contrast due to the complex and intricate interplay of light, water, and objects. Despite the significant contributions of previous underwater enhancement techniques, there exist several problems that demand further improvement: (i) The current deep learning methods rely on Convolutional Neural Networks (CNNs) that lack the multi-scale enhancement, and global perception field is also limited. (ii) The scarcity of paired real-world underwater datasets poses a significant challenge, and the utilization of synthetic image pairs could lead to overfitting. To address the aforementioned problems, this paper introduces a Multi-scale Transformer-based Network called UWFormer for enhancing images at multiple frequencies via semi-supervised learning, in which we propose a Nonlinear Frequency-aware Attention mechanism and a Multi-Scale Fusion Feed-forward Network for low-frequency enhancement. Besides, we introduce a special underwater semi-supervised training strategy, where we propose a Subaqueous Perceptual Loss function to generate reliable pseudo labels. Experiments using full-reference and non-reference underwater benchmarks demonstrate that our method outperforms state-of-the-art methods in terms of both quantity and visual quality.

==> figtex/2_model.tex <==
\begin{figure*}[ht]
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{1.0\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Semi.pdf}}
        \end{minipage}
    \end{minipage}
    \caption{
    Proposed underwater semi-supervised training strategy of ours. Labeled images $X_l \in \mathbb{R}^{C \times H \times W}$ and unlabeled images $X_u \in \mathbb{R}^{C \times H \times W}$ are be fed to:(i) the student model for training, and (ii) the teacher model for unlabeled prediction. The student model outputs labeled rewhile augmented unlabeled images $X_{ua}$ will be fed into the student model for unlabeled prediction. The student model outputs labeled results $\hat{X_l}$ and unlabeled results $\hat{X_u}$, with the $\hat{X_l}$ converging using a supervised loss function. Note that the outputs of the teacher model are evaluated and updated in real-time using UCIQE to generate positive samples $X_p$. Finally, the unlabeled outputs of the student model $\hat{X_u}$ are constrained by $X_p$ using an unsupervised loss function. In this case, the weights of the student model are determined by both labeled data and  unlabeled data.
    } 
    \label{fig:model}
\end{figure*}

==> figtex/AFF.tex <==
\begin{figure}[ht]
    \begin{minipage}[b]{0.9\linewidth}
        \includegraphics[width=\linewidth]{figs/AFF.pdf}
    \end{minipage}
    \caption{
    The structures of sub-modules: (a) Feature Extraction, (b) Asymmetric Feature Fusion
    }
    \label{fig:aff}
\end{figure}




==> figtex/teaser.tex <==
\begin{teaserfigure}
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/teaser/input.jpg}}
            \centerline{(a) Input}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/teaser/mmle.jpg}}
            \centerline{(b) MMLE}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/teaser/ucolor.jpg}}
            \centerline{(c) Ucolor}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/teaser/ours.jpg}}
            \centerline{(d) Ours}\medskip
        \end{minipage}
        \begin{minipage}[b]{0.19\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/teaser/target.jpg}}
            \centerline{(e) Target}\medskip
        \end{minipage}
    \end{minipage}
    \caption{The figure illustrates a comparison between degraded underwater image (a) and its restored version (e) obtained from the EUVP dataset. Although traditional enhancement techniques (b) and deep learning models (c) have been employed, they still manifest imperfections. By contrast, our method (d) effectively enhances the image.}
    \label{fig:teaser}
\end{teaserfigure}


==> tables/noref_ab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\centering
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
{ }                         & \multicolumn{2}{c|}{{ EUVPUN}}                             & \multicolumn{2}{c|}{{ U45}}                                & \multicolumn{2}{c|}{{ RUIE}}                               & \multicolumn{2}{c|}{{ UIEB-60}}                            \\ \cline{2-9} 
\multirow{-2}{*}{{ Method}} & { UIQM$\uparrow$} & { UCIQE$\uparrow$} & { UIQM$\uparrow$} & { UCIQE$\uparrow$} & { UIQM$\uparrow$} & { UCIQE$\uparrow$} & { UIQM$\uparrow$} & { UCIQE$\uparrow$} \\ \hline
{ UNet}                     & { 2.485}          & { 0.395}           & { 2.936}          & { 0.378}           & { 2.481}          & { 0.247}           & { 2.406}          & { 0.351}           \\
{ W/O SPL}              & { }          & { }           & { }          & { }           & { }          & { }           & { }          & { }           \\
{ MDTA+MSFN}           & { 2.723}          & { 0.408}           & { 3.101}          & { 0.401}           & { 2.686}          & { 0.315}           & { 2.711}          & { 0.361}           \\
{ NFA+GDFN}             & { 2.710}          & { 0.403}           & { 3.043}          & { 0.396}           & { 2.711}          & { 0.312}           & { 2.713}          & { 0.391}           \\
{ Supervised}               & { 2.658}          & { 0.419}           & { 3.136}          & { 0.403}           & { 2.781}          & { 0.314}           & { 2.718}          & { 0.377}           \\ \hline
{ Ours}                     & {\color[HTML]{DE3C36} \textbf{2.826}} & {\color[HTML]{DE3C36} \textbf{0.441}}  & {\color[HTML]{DE3C36} \textbf{3.192}} & {\color[HTML]{DE3C36} \textbf{0.438}}  & {\color[HTML]{DE3C36} \textbf{2.887}} & {\color[HTML]{DE3C36} \textbf{0.346}}  & {\color[HTML]{DE3C36} \textbf{2.786}} & {\color[HTML]{DE3C36} \textbf{0.415}}  \\ \hline
\end{tabular}
\caption{Quantitative results of ablation studies on no-reference datasets}
\label{tab:noref_ab}
\end{table*}

==> tables/ref_ab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\centering
\begin{tabular}{|c|cccc|cccc|}
\hline
{\color[HTML]{000000} }                         & \multicolumn{4}{c|}{{\color[HTML]{000000} UIEB}}                                                                                                                                                                                 & \multicolumn{4}{c|}{{\color[HTML]{000000} EUVP}}                                                                                                                                                                                 \\ \cline{2-9} 
\multirow{-2}{*}{{\color[HTML]{000000} Method}} & \multicolumn{1}{c|}{{\color[HTML]{000000} PSNR$\uparrow$}} & \multicolumn{1}{c|}{{\color[HTML]{000000} SSIM$\uparrow$}} & \multicolumn{1}{c|}{{\color[HTML]{000000} LPIPS$\downarrow$}} & {\color[HTML]{000000} UCIQE$\uparrow$} & \multicolumn{1}{c|}{{\color[HTML]{000000} PSNR$\uparrow$}} & \multicolumn{1}{c|}{{\color[HTML]{000000} SSIM$\uparrow$}} & \multicolumn{1}{c|}{{\color[HTML]{000000} LPIPS$\downarrow$}} & {\color[HTML]{000000} UCIQE$\uparrow$} \\ \hline
{\color[HTML]{000000} UNet}                     & {\color[HTML]{000000} 17.93}                               & {\color[HTML]{000000} 0.792}                               & {\color[HTML]{000000} 0.200}                                  & {\color[HTML]{000000} 0.389}           & {\color[HTML]{000000} 22.19}                               & {\color[HTML]{000000} 0.802}                               & {\color[HTML]{000000} 0.212}                                  & {\color[HTML]{000000} 0.384}           \\
{\color[HTML]{000000} W/O SPL}              & {\color[HTML]{000000} }                               & {\color[HTML]{000000}}                               & {\color[HTML]{000000} }                                  & {\color[HTML]{000000} }           & {\color[HTML]{000000} }                               & {\color[HTML]{000000} }                               & {\color[HTML]{000000} }                                  & {\color[HTML]{000000} }       \\
{\color[HTML]{000000} MDTA+MSFN}           & {\color[HTML]{000000} 21.26}                               & {\color[HTML]{000000} 0.830}                               & {\color[HTML]{000000} 0.140}                                  & {\color[HTML]{000000} 0.402}           & {\color[HTML]{000000} 24.18}                               & {\color[HTML]{000000} 0.823}                               & {\color[HTML]{000000} 0.151}                                  & {\color[HTML]{000000} 0.411}           \\
{\color[HTML]{000000} NFA+GDFN}             & {\color[HTML]{000000} 21.82}                               & {\color[HTML]{000000} 0.826}                               & {\color[HTML]{000000} 0.144}                                  & {\color[HTML]{000000} 0.439}           & {\color[HTML]{000000} 22.56}                               & {\color[HTML]{000000} 0.740}                               & {\color[HTML]{000000} 0.191}                                  & {\color[HTML]{000000} 0.425}           \\
{\color[HTML]{000000} Supervised}               & {\color[HTML]{000000} 22.72}                               & {\color[HTML]{000000} 0.894}                               & {\color[HTML]{000000} 0.085}                                  & {\color[HTML]{000000} 0.413}           & {\color[HTML]{000000} 24.24}                               & {\color[HTML]{000000} 0.840}                               & {\color[HTML]{000000} 0.155}                                  & {\color[HTML]{000000} 0.411}           \\ \hline
{\color[HTML]{000000} Ours}                     & {\color[HTML]{DE3C36} \textbf{23.25}}                      & {\color[HTML]{DE3C36} \textbf{0.904}}                      & {\color[HTML]{DE3C36} \textbf{0.075}}                         & {\color[HTML]{DE3C36} \textbf{0.446}}  & {\color[HTML]{DE3C36} \textbf{24.41}}                      & {\color[HTML]{DE3C36} \textbf{0.846}}                      & {\color[HTML]{DE3C36} \textbf{0.129}}                         & {\color[HTML]{DE3C36} \textbf{0.432}}  \\ \hline
\end{tabular}
\caption{Quantitative results of ablation studies on full-reference datasets}
\label{tab:ref_ab}
\end{table*}



==> tables/userstudy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\begin{tabular}{|c|cc|}
\hline
{\color[HTML]{000000} }                         & \multicolumn{1}{c|}{{\color[HTML]{000000} Full-reference}} & {\color[HTML]{000000} No-reference} \\ \cline{2-3} 
\multirow{-2}{*}{{\color[HTML]{000000} Method}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Ranking}}        & {\color[HTML]{000000} Ranking}      \\ \hline
{\color[HTML]{000000} FunieGAN}                 & {\color[HTML]{000000} 2.00}                                    & {\color[HTML]{000000} 1.57}             \\
{\color[HTML]{000000} Ucolor}                   & {\color[HTML]{000000} 2.88}                                    & {\color[HTML]{000000} 3.00}             \\
{\color[HTML]{000000} PWRNet}                   & {\color[HTML]{000000} 4.00}                                    & {\color[HTML]{000000} 4.00}             \\ \hline
{\color[HTML]{000000} Ours}                     & {\color[HTML]{DE3C36} \textbf{1.12}}                           & {\color[HTML]{DE3C36} \textbf{1.42}}    \\ \hline
\end{tabular}
\caption{The user study conduct on full-reference and no-reference datasets ranked several methods, and the results are averaged to determine the rankings. A lower ranking indicates better human subjective evaluation.
}
\label{tab:user}
\end{table}



